Wonderland: Navigating 3D Scenes from a Single Image

How can one efficiently generate high-quality, wide-scope 3D scenes from arbitrary single images? Existing methods suffer several drawbacks, such as requiring multi-view data, time-consuming per-scene optimization, distorted geometry in occluded areas, and low visual quality in backgrounds. Our novel 3D scene reconstruction pipeline overcomes these limitations to tackle the aforesaid challenge. Specifically, we introduce a large-scale reconstruction model that leverages latents from a video diffusion model to predict 3D Gaussian Splattings of scenes in a feed-forward manner. The video diffusion model is designed to create videos precisely following specified camera trajectories, allowing it to generate compressed video latents that encode multi-view information while maintaining 3D consistency. We train the 3D reconstruction model to operate on the video latent space with a progressive learning strategy, enabling the efficient generation of high-quality, wide-scope, and generic 3D scenes. Extensive evaluations across various datasets affirm that our model significantly outperforms existing single-view 3D scene generation methods, especially with out-of-domain images. Thus, we demonstrate for the first time that a 3D reconstruction model can effectively be built upon the latent space of a diffusion model in order to realize efficient 3D scene generation.

==> table/notation.tex <==

%=================================================
%=================================================
\begin{table*}
\centering
\caption{\textbf{Mathematical notation used in the paper.}}
\label{Tab:notation}
\begin{tabular}{lll}
\toprule
\textbf{Expression} & \textbf{Specification} & \textbf{Explanation} \\
\midrule
\textit{commonly used} & \multicolumn{2}{c}{}  \\
$x$ & $x\in R^{T\times H\times W\times 3}$ & source video clip \\
$s$ & - & stride to sample clip $x$ from source video \\
% $T$,$H$,$W$ & 49,480,720 & temporal length, height, width of $x$ \\
$z$ & $z \in R^{t\times h\times w\times c}$ & video latent embedded from $x$ \\
$\mathcal{E}$ & - & encoder from 3D-VAE \\
$r_s$ & $r_s=\frac{H}{h}=\frac{W}{w}$ & spatial compression rate \\[3pt]
$r_t$ & $r_t=\frac{T}{t}$ & temporal compression rate \\[3pt]
$p$ & $p \in R^{T\times H\times W\times 6}$ & Plücker embedding of cameras of video clip $x$ \\
\midrule
\textit{diffusion related} & \multicolumn{2}{c}{}  \\
$\tau$ & - & diffusion time step \\
$\alpha_{\tau}, \sigma_{\tau}$ & - & diffusion noise scheduler parameters \\
$\epsilon$ & $\epsilon \in R^{t\times h\times w\times c}$ & random noise where $\epsilon \sim \mathcal{N}(0,I)$ \\
$z_\tau$ & $z_\tau \in R^{t\times h\times w\times c}$ & noisy video latent \\
$D_{\theta}$ & - & diffusion model parameterized by $\theta$ \\
$y$ & - & conditional signal, usually textual embedding \\
$o_v$ & $o_v\in R^{N_v\times d_v}$ & visual tokens as a sequence in diffusion model \\
$o_\mathrm{ctrl}$, $o_\mathrm{lora}$ & $o_\mathrm{ctrl}$, $o_\mathrm{lora}$ $\in R^{N_v\times d_v}$ & camera tokens as a sequence in diffusion model \\
$N$ & - & number of transformer blocks in ControlNet branch \\
\midrule
\textit{reconstruction related} & \multicolumn{2}{c}{}  \\
$p_l$ & - & spatial patch size applied to $z$ in LaLRM \\
$o_l$ & $o_l\in R^{N_l\times d_l}$ & visual latent tokens as a sequence in LaLRM \\
$N_l$ & $N_l=t\cdot \frac{h}{p_l}\cdot \frac{w}{p_l}$ & number of visual latent tokens in LaLRM \\[5pt]
$o_\mathrm{p}$ & $o_\mathrm{p}$ $\in R^{N_l\times d_l}$ & camera tokens as a sequence in LaLRM \\
$V$ & - & number of supervision views in LaLRM \\
$G$ & $G\in R^{(T\cdot H\cdot W)\times 12}$ & Gaussian feature map in LaLRM \\
\bottomrule
\end{tabular}
\end{table*}
%=================================================
%==============================
